On The Sample Complexity Bounds In Bilevel Reinforcement Learning

Bilevel reinforcement learning (BRL) has emerged as a powerful framework for aligning generative models, yet its theoretical foundations, especially sample complexity bounds, remain underexplored. In this work, we present the first sample complexity bound for BRL, establishing a rate of $\mathcal{O}(\epsilon^{-3})$ in continuous state-action spaces. Traditional MDP analysis techniques do not extend to BRL due to its nested structure and non-convex lower-level problems. We overcome these challenges by leveraging the Polyak-{\L}ojasiewicz (PL) condition and the MDP structure to obtain closed-form gradients, enabling tight sample complexity analysis. Our analysis also extends to general bi-level optimization settings with non-convex lower levels, where we achieve state-of-the-art sample complexity results of $\mathcal{O}(\epsilon^{-3})$ improving upon existing bounds of $\mathcal{O}(\epsilon^{-6})$. Additionally, we address the computational bottleneck of hypergradient estimation by proposing a fully first-order, Hessian-free algorithm suitable for large-scale problems.

==> figures_tex/reward_results.tex <==
% \begin{figure}[H]
% \centering
% \includegraphics[width=0.49\linewidth]{figures/comparison_walker.pdf}
% \includegraphics[width=0.49\linewidth]{figures/comparison_dooropen.pdf}
% %\vspace{-5mm}
% \caption{Training curves on Walker locomotion task (left) from the DeepMind Control Suite~\cite{tassa2018deepmind} and the Door Open manipulation task (right) from Meta-world~\cite{mclean2025metaworld}. The solid line and shaded regions respectively denote mean and standard deviation of success rate, across multiple seeds. Blue curve: PEBBLE, Red curve: OURS.}
% \label{fig:reward_ablation}
% \end{figure}
